Evaluating and Improving Context Attention Distribution on Multi-Turn Response Generation using Self-Contained Distractions

Despite the rapid progress of open-domain generation-based conversational agents, most deployed systems treat dialogue contexts as single-turns, while systems dealing with multi-turn contexts are less studied. There is a lack of a reliable metric for evaluating multi-turn modelling, as well as an effective solution for improving it. In this paper, we focus on an essential component of multi-turn generation-based conversational agents: context attention distribution, i.e. how systems distribute their attention on dialogue's context. For evaluation of this component, We introduce a novel attention-mechanism-based metric: DAS ratio. To improve performance on this component, we propose an optimization strategy that employs self-contained distractions. Our experiments on the Ubuntu chatlogs dataset show that models with comparable perplexity can be distinguished by their ability on context attention distribution. Our proposed optimization strategy improves both non-hierarchical and hierarchical models on the proposed metric by about 10% from baselines.

==> input/conclusion.tex <==
We have studied context attention distribution, an essential component of multi-turn modelling for open-domain conversational agents. We have proposed an evaluation metric for context attention distribution based on the distracting test: DAS ratio. We have also improved the performance of context attention distribution for common multi-turn conversational agents through an optimization strategy via reducing the attention loss of self-contained distracting utterances. Extensive experiments show that our proposed strategy achieves improvements on most models, especially with a training inserting probability level of $0.7$. Future works can focus on adapting the proposed evaluation metric and optimization strategy to transformer-based conversational agents.

% We have applied our proposed evaluation metric to $23$ model variants on $9$ different distracting test sets. 
